Rethinking Bradley-Terry Models in Preference-Based Reward Modeling: Foundations, Theory, and Alternatives

The Bradley-Terry (BT) model is a common and successful practice in reward modeling for Large Language Model (LLM) alignment. However, it remains unclear why this model -- originally developed for multi-player stochastic game matching -- can be adopted to convert pairwise response comparisons to reward values and make predictions. Especially given the fact that only a limited number of prompt-response pairs are sparsely compared with others. In this paper, we first revisit the foundations of using BT models in reward modeling, and establish the convergence rate of BT reward models based on deep neural networks using embeddings, providing a theoretical foundation for their use. Despite theoretically sound, we argue that the BT model is not a necessary choice from the perspective of downstream optimization. This is because a reward model only needs to preserve the correct ranking predictions through a monotonic transformation of the true reward. We highlight the critical concept of order consistency in reward modeling and demonstrate that the BT model possesses this property. Consequently, we propose a simple and straightforward upper-bound algorithm, compatible with off-the-shelf binary classifiers, as an alternative order-consistent reward modeling objective. To offer practical insights, we empirically evaluate the performance of these different reward modeling approaches across more than 12,000 experimental setups, using $6$ base LLMs, $2$ datasets, and diverse annotation designs that vary in quantity, quality, and pairing choices in preference annotations.

==> tex/sec_bradleyterry.tex <==
\section{Background: LLM Alignment and the Bradley-Terry Model}
The alignment of Large Language Models (LLMs) is crucial for their safe and effective deployment across various applications. Current research on reinforcement learning from human feedback (RLHF)~\citep{christiano2017deep,stiennon2020learning,ouyang2022training} has largely focused on utilizing offline, preference-based annotations provided by humans or general-purpose LLMs~\cite{bai2022constitutional,lee2023rlaif,guo2024direct}. 
Due to the substantial costs associated with gathering consistent human annotations, RLHF research has predominantly concentrated on an off-policy, offline setting~\footnote{Here, the \textit{Off-Policy} refers to generating pairwise responses using a language model, $\llm_{\mathrm{off}}$, distinct from the model, $\llm_{\mathrm{on}}$ to be aligned. The \textit{Offline} refers to that annotators do not interact in real-time and further engagements are not permitted.
}.

The data generation process of the preference annotation starts with a pre-collected prompt dataset $\dataset{prompt} = \{\prompt_\dataidx\}_{\dataidx\in [n]}$, comprising $N$ prompts from a uniform domain, such as a compilation of potential user queries to an AI assistant. Responses are generated in pairs using $\llm_{\mathrm{off}}$: $\response_1,\response_2 \sim \llm_\mathrm{off}(\prompt)$, followed by human annotation for each pair $\preff$, being -1 if $\response_{1}$ if preferred and 1 otherwise. This dataset is formally represented as triples, $\dataset{pref} = \{(\prompt_\dataidx, \response_{1,\dataidx}, \response_{2,\dataidx}, \preff_{\dataidx})\}_{\dataidx \in [n]}$, where $\prompt_\dataidx$ denotes the prompt, and $ \response_{1,\dataidx}, \response_{2,\dataidx}$ indicate the responses and $\preff_{\dataidx}$ preference according to annotation.

With the above dataset, there are two primary approaches to RLHF: Direct policy optimization \citep{rafailov2024direct, zhao2023slic, azar2023general}, which achieves LLM alignment through a straightforward supervised learning objective, and the alternate method that constructs a reward model to guide the LLM optimization via either supervised learning or reinforcement learning \citep{yuan2023rrhf, dong2023raft, munos2023nash, li2023remax}. Among these different strategies, the majority of them, including those employed in large-scale alignment tasks, rely on the Bradley-Terry model \citep{bradley1952rank} to translate pairwise comparisons into scores, thereby constructing objectives for LLM optimization.\footnote{In the standard application of the Bradley-Terry model, pairwise competition results are converted into definitive scores reflecting the players' capabilities.}

% Despite differences in LLM alignment strategies, the majority of these methods --- including some of the most successful algorithms deployed for large-scale alignment tasks --- assume the Bradley-Terry model~\citep{bradley1952rank} to either explicitly or implicitly convert pairwise comparisons into scores, which are then used as objectives for the LLM to optimize.\footnote{In the standard application of the Bradley-Terry model, pairwise competition outcomes are converted into absolute scores that represent the players' abilities.}


Although the Bradley-Terry model has achieved empirical success in alignment practices, the rationale behind its application remains ambiguous. As we will elaborate below, the problem setup for offline RLHF differs significantly from the conventional application of the Bradley-Terry model in multi-player games. To clarify this, we will begin by revisiting the fundamental assumptions and intuitions of the Bradley-Terry model and then present a case study in the LLM arena that illustrates its more explicit application within the LLM context.

\paragraph{A Historical Account}
Hark back to the seminal paper on RLHF~\citep{christiano2017deep}, the motivation for using the Bradley-Terry-\textit{type} model is to understand it as a specialization of the Luce-Shephard choice rule~\citep{luce1959individual,shepard1957stimulus}. In a simplified version of the two-option setting, the Luce-Shephard choice rule says the \textbf{probability} of choosing a particular option $i$ from a set of alternatives $\{i,j\}$ is proportional to the utility $\truereward(\cdot)$ assigned to that option. Formally, 
\begin{equation}
\label{eqn:bradley-terry}
    P(i~\text{winning}|i,j \text{ competing}) = \frac{\truereward(i)}{\truereward(i)+\truereward(j)}.
\end{equation}
The application of such a rule is well aligned with the Bradley-Terry model~\cite{bradley1952rank} where pairwise comparisons between players can be used to estimate their ability (utility) scores, where a game is inherently stochastic while the ability of a player is fixed. In later work of alignment from human feedback~\cite{stiennon2020learning,ouyang2022training,rafailov2023direct}, such a model is directly applied and has achieved great success in improving the quality of LLMs in various tasks when direct evaluation is impossible.

The usage of the Bradley-Terry model in RLHF has been challenged in the literature from different perspectives: \cite{munos2023nash} points that the Bradley-Terry model can not capture non-transitive preferences, and maximizing the corresponding Elo score can be a different objective as compared to the objective of optimizing preferences. 
\cite{azar2023general} points out that using the Bradley-Terry modelization in the direct preference optimization methods~\citep{rafailov2023direct} could lead to problematic overfitting when sampled preferences are deterministic. 





\section{Two use Cases of the Bradley-Terry Model: LLM arena vs reward modeling}
In the following, we discuss two key applications of the Bradley-Terry model in ranking systems for LLMs to better contrast the difference between its conventional application and un-natural application in RLHF.
\paragraph{The Bradley-Terry Model in Online LLM Arenas: Direct Parameterization and MLE}
One of the successful usages of the Bradley-Terry Model model is in the LLM chatbot arena \cite{chiang2024chatbot}, where different LLMs compete against each other through paired comparisons according to human feedback. In such a process, each LLM is a player, and human-annotated preferences represent the results of games. Importantly, those LLM players play \textbf{many games} to estimate the precise ability of each \textit{LLM} --- there are about 130 models, and more than 1,700,000 comparisons have been made --- on average, each model has played against other models on more than 26,000 games.

Consider a set of \(\totalllms\) LLMs, each denoted by \(\llm_\llmidx\) for \(\llmidx = 1, 2, \dots, \totalllms\). Each LLM has an associated ability score \(S_\llmidx \in \mathbb{R}\), which represents its overall performance in generating responses as evaluated by users.
Suppose that \(n\) pairwise comparisons are conducted, where in each comparison, two LLMs, say \(\llm_\llmidx\) and \(\llm_j\), are evaluated. Let \(\preff_\dataidx = 1\) if \(\llm_\llmidx\) is preferred over \(\llm_j\) in the \(\dataidx\)-th comparison, and \(\preff_\dataidx = 0\) otherwise, for \(\dataidx = 1, 2, \dots, n\).
The Bradley-Terry model posits that the probability \(p_{ij}\) that \(\llm_\llmidx\) is preferred over \(\llm_j\) is given by:
\begin{equation}
     p_{\llmidx j} = P(\llm_\llmidx \succ \llm_j) = \frac{1}{1 + e^{-(S_\llmidx - S_j)}}   
\end{equation}
Given the outcomes \(\preff_1, \preff_2, \dots, \preff_\dataidx\) of the \(n\) comparisons, the likelihood function for the parameters \(S_1, S_2, \dots, S_\totalllms\) is:
\begin{equation}
\mathcal{L}(S_1, S_2, \dots, S_\totalllms) = \prod_{\dataidx=1}^n p_{\llmidx_\dataidx j_\dataidx}^{\preff_\dataidx} \cdot (1 - p_{\llmidx_\dataidx j_\dataidx})^{1 - \preff_\dataidx}
\end{equation}
where \(p_{\llmidx_\dataidx j_\dataidx}\) is the probability that \(\llm_{\llmidx_\dataidx}\) is preferred over \(\llm_{j_\dataidx}\) in the \(\dataidx\)-th comparison, given by:
\begin{equation}
p_{\llmidx_\dataidx j_\dataidx} = \frac{1}{1 + e^{-(S_{\llmidx_\dataidx} - S_{j_\dataidx})}}
\end{equation}
The log-likelihood function is then:
\begin{equation}
    \begin{split}
        \ell_n(\mathbf{S}) = \ell_n(S_1, S_2, \dots, S_\totalllms) &= \sum_{\dataidx=1}^n \left[ \preff_\dataidx \log p_{\llmidx_\dataidx j_\dataidx} + (1 - \preff_\dataidx) \log(1 - p_{\llmidx_\dataidx j_\dataidx}) \right] \\
        &= \sum_{\dataidx=1}^n \left[ \preff_\dataidx (S_{\llmidx_\dataidx} - S_{j_\dataidx}) - \log(1 + e^{S_{\llmidx_\dataidx} - S_{j_\dataidx}}) \right]
    \end{split}
\end{equation}

The maximum likelihood estimates (MLE) of the parameters \(S_1, S_2, \dots, S_\totalllms\) are obtained by maximizing the log-likelihood function:
\begin{equation}
\hat{\mathbf{S}}_n = \hat{S}_1, \hat{S}_2, \dots, \hat{S}_\totalllms = \arg\max_{S_1, S_2, \dots, S_\totalllms} \ell(S_1, S_2, \dots, S_\totalllms)
\end{equation}
we have the following consistency result:
% \begin{restatable}[Average Order Consistency of Annotation]{proposition}{PropAvgQuality}
% \label{prop:1}
%\ys{I think we can put this in appendix, as it is a known result}
\begin{restatable}[Consistency of MLE for Bradley-Terry Model \citet{ford1957solution,wu2022asymptotic}]{theorem}{TheoremOne}
\label{theorem:1.1}
    Let \( \hat{\mathbf{S}}_n = (\hat{S}_1, \hat{S}_2, \dots, \hat{S}_\totalllms) \) be the Maximum Likelihood Estimator (MLE) for the ability scores \( \mathbf{S} = (S_1, S_2, \dots, S_\totalllms) \) in the Bradley-Terry model based on \( n \) pairwise comparisons between each pair. We further assume $S_1=0$, Assume that the true ability scores \( \mathbf{S}^* = (S_2, \dots, S_\totalllms) \) are distinct and that the comparisons \( \preff_\dataidx \) are independent according to the model. Then, \( \hat{\mathbf{S}}_n \) is a consistent estimator of \( \mathbf{S}^* \), i.e.,
\begin{equation}
    \hat{\mathbf{S}}_n \xrightarrow{P} \mathbf{S}^* \quad \text{as } n \rightarrow \infty.
\end{equation}
\end{restatable}

%\jef{do we really need infinity?. how about all pairwise comparisons?} \hs{there is a tightened theorem~\cite{han2020asymptotic} saying after we have $n*(\log n)^3$ comparisons, we could have a consistent estimation.}



% Setting these partial derivatives to zero, we get the overparameterization problem. \hs{identifiability}

\paragraph{The Bradley-Terry Model in LLM Alignment: The Sparsity and Re-Parameterization.}
In the context of RLHF, the high-level motivation of using the Bradley-Terry model is to convert \textbf{pairs of preference-based data into scores}. In this process, different responses are treated as players, and human evaluations are considered to be \textit{noisy}\footnote{In the literature, the source of this noisy annotation is ambiguous.}. 
In contrast to LLM arena where we want a score for each \textit{LLM} that are \textit{seen}, here we want a much more fine grained score for each \textit{prompt-response} pairs and the ability to predict it for \textit{unseen} pairs.
To define the game, we need to first clarify the following concepts and definitions:
\begin{definition}[Oracle Utility function $\truereward$]
    We assume there exist an oracle utility value $\truereward \mathcal{X}\times \mathcal{Y} \to \mathbb{R}$ for all prompt-response pairs. This value manifest the alignment of the response with respect to the desired objective. e.g., helpfulness of an AI chatbot.
\end{definition}
\begin{assumption}[Stochasticity Source in Preference Annotations as a Match]
    We assume the noise in making observations to the pairwise comparison originates from the random biases in human annotators' evaluations. We use $\annotatorbias(\cdot, \cdot|\omega):\mathcal{X}\times \mathcal{Y}\mapsto \mathbb{R}$ to denote those annotation biases as random variables. In comparing $\prompt, \response_{1}$ and $\prompt, \response_{2}$, the human annotation $h:\mathcal{X}\times\mathcal{Y}\times\mathcal{Y}\mapsto \Delta\{-1,1\}$ is instantiated through the following comparison:
    \begin{equation}
   h(\prompt,\response_{1},\response_{2}|\omega) = 
    \begin{cases} 
  1, & \text{if }~~ \truereward(\prompt,\response_{1})+\annotatorbias(\prompt,\response_{1}|\omega)\ge \truereward(\prompt,\response_{2})+\annotatorbias(\prompt,\response_{2}|\omega),\\
  -1, & \text{otherwise}
\end{cases}
    \end{equation}
    Moreover, to apply the Bradley-Terry model, we need further \textbf{assume the players' ability differences are sampled from a logistic distribution}, then the probability of preference is given as a logistic regression over utility difference, 
    \begin{equation}
        P(\response_{1}\succ \response_{2}) = \frac{1}{1+e^{-(\truereward(\prompt,\response_{1}) - \truereward(\prompt,\response_{2}))}}
    \end{equation}
\end{assumption}
Basically, this means that human annotators can provide consistent (deterministic) annotations, i.e., If annotators are asked to rank the same pair of responses multiple times, their annotation should remain consistent, reflecting their persistent belief on the quality of different responses. 
% \begin{assumption}[Stochasticity Source in Preference Annotations as a Match]
%     It is important to note that the source of stochasticity arises from randomized annotation \textbf{biases} rather than the inherent randomness in individual annotations. Different annotators may have their individual biases towards responses, but these biases are consistent across multiple evaluations. 
% \end{assumption}
%We note that the above Assumption can always be true if we only work with consistent annotations and annotators.
%\begin{definition}[\textcolor{red}{Unbiased Preference over Population}]
%    We define the oracle utility function to be the population level expectation of the biased evaluation of different responses. i.e.,
%    \begin{equation}
%        \mathbb{E}_{\omega}\annotatorbias(\prompt,y|\omega) = 0, \forall \prompt, y
%    \end{equation}
%\end{definition}

\begin{comment}
\paragraph{Requirements for Localized Consistent Utility Estimation}
We now introduce an ideal setting where we can seamlessly apply the Bradley Terry Model. In this setting, we use the language model $\llm_\mathrm{off}$ to generate $K$ responses $\{y^{(i)}_\totalllms \}_{k\in[K]} \sim \llm_\mathrm{off}$ to each of the queries $x_i, i\in[N]$, and let \textbf{a group of annotators} to annotate their preferences over different pairs of responses given a question. We use $r^*_{i,k}$ to denote the ability (oracle utility value) of the $k$-th player $y_\totalllms^{(i)}$ given the prompt $x_i$. Then we have


\begin{corollary}[Locally Consistent Utility Estimators]
    Let \( \hat{\mathbf{r}}^{(i)}_n = (\hat{r}_{i,1}, \hat{r}_{i,2}, \dots, \hat{r}_{i,k}) \) be the Maximum Likelihood Estimator (MLE) for the ability scores \( \mathbf{r} = (\truereward_{i,1}, \truereward_{i,2}, \dots, \truereward_{i,k}) \) in the Bradley-Terry model based on \( n \) pairwise comparisons. Assume that the true ability scores \( \mathbf{r}^*_i = (r^*_{i,1}, r^*_{i,2}, \dots, r^*_{i,K}) \) are identifiable and that the comparisons \( h \) are independent and identically distributed (i.i.d.) according to the model. Then, \( \hat{\mathbf{r}}^{(i)}_n \) is a consistent estimator of \( \mathbf{r}^* \), i.e.,
\begin{equation}
    \hat{\mathbf{r}}^{(i)}_n \xrightarrow{P} \mathbf{r}^*_i \quad \text{as } n \rightarrow \infty.
\end{equation}
\end{corollary}

This means that with sufficient annotations on each pair of responses, we are able to accurately estimate their true ability scores up to a constant (due to the identifiability issue). 
\end{comment}

\paragraph{Global Reward Model as Universal Utility Approximator}
However, in practice, each pair of players typically competes only once. When we have $N$ prompts, this practice lead to $K = 2N$ responses as players, and we have in total $n=N$ comparisons.  The number of comparisons is only half the number of the players. If these comparisons happen in random following Erd\"os–R\'enyi model, on average one need at least on average $N\log(N)$ comparisons \citep{han2020asymptotic} and even if one have access to true utility scores, with quick sort one needs on average $N\log(N)$ comparisons. Therefore, it is likely impossible to solve the estimation problem~\citep{han2020asymptotic} and it is impractical to directly parameterize the scores of each players (response). More over, even if we have enough comparisons like in arena setting, it is unclear how we could make predictions on unseen prompt-response pairs when we directly parameterize reward, a crucial task for RLHF. Given such sparsity of annotation, the literature has proposed to build a parameterized \textbf{reward model} $R_\theta: \mathcal{X}\times\mathcal{Y}\mapsto\mathbb{R}$ to re-parameterize the players' abilities as a Universal Utility Approximator~\citep{christiano2017deep,ouyang2022training,rafailov2023direct,dong2023raft}.

%\hs{e.g., if we are working on a deterministic sorting, the sample complexity will be nlogn. without further assumption, it's generally impossible to do parameter estimation with less than nlogn comparisons. (the theoretical lower bound for consistent estimation in the literature is nlogn)}

Under the generic form of the Bradley-Terry model, the probability of observing response \( \response_A \) being preferred over response \( \response_B \) given prompt \( \prompt \) is expressed as:
\begin{equation}
\label{eqn:re-parameterization}
    % P(\response_A \succ \response_B|\prompt) = \frac{1}{2} + \frac{1}{2}\mathrm{tanh}\left(\frac{r_A-r_B}{\sqrt{2(v_A^2 + v_B^2)}}\right)
    P(\response_A \succ \response_B|\prompt, R_\theta(\prompt,\response_A) - R_\theta(\prompt,\response_B)) = \sigma(R_\theta(\prompt,\response_A) - R_\theta(\prompt,\response_B)),
\end{equation}
%\ys{the left hand side is not a function of $y_A,y_B$ while the right hand side is. I'm quite sure you mean something else }
and solved through maximum likelihood.
% In this application, it is impractical to directly parameterize the scores of each player (response), as the number of players corresponds to the number of responses. Given the sparsity of annotations—each pair of responses typically receives only a single annotation—and the fact that as \( M \) (the number of pairs) approaches infinity, the number of players also increases to infinity, it becomes necessary to build a parameterized model to re-parameterize the players' abilities.

%\begin{equation}
%\widetilde{\mathcal{L}}_\mathrm{CE} = -\mathbb{E}_{(\prompt,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}}\left[\log \sigma 
% \small 
%\left(R_\theta(\prompt, y^+) - R_\theta(\prompt, y^-)\right)\right]
%\end{equation}

However, since we are never going to observe the comparison for multiple times, we are not actually working under the setting that the Bradley-Terry model is built to handle. In this case, the following important questions arises:
\begin{enumerate}[nosep]
    \item Can the objective based on the Bradley-Terry model be used to learn reward?
    \item Is the objective based on the Bradley-Terry model a necessary choice for RLHF?
    \item Why is the probability notation in \eqref{eqn:re-parameterization} still meaningful and helpful?
    \item Could we instead use other models such as the binary classification model? 
    \item Given the fact that the reward model is a universal utility approximator, what would be the optimal data format and optimization objective? 
\end{enumerate}  

In the next section, we answer those questions by introducing the order consistency objective in reward modeling. We will work without the Bradley-Terry model as the prior assumption over preference data and ability scores. 

\hs{so the only thing we can do is to build a regression model with partial pairwise comparisons (partially observable).}

%\section{\textcolor{red}{To Make BT-Model Work, How to Fix with Embeddings?}}


==> tex/sec_derivingBT.tex <==
\section{Underlying Assumptions of Applying the Bradley-Terry Model in Preference Annotations}
\label{appdx:implication_of_assumptions}
%\ys{can we say this is rederiving this model from cognitive bottle neck or something indicating we start from human bias rather than random game?}
Different from those prior works that challenge the \textit{practical application} of the BT model~\cite{azar2023general,munos2023nash,tang2024generalized}, we revisit the basic assumptions of modeling human preference annotations with the BT model, and answer the following questions:

\textbf{\textit{What are the underlying assumptions when we assume the BT model can be used to model the preference annotations?}}

The canonical interpretation of how to apply \eqref{eqn:BT} in preference-based learning is that: when randomly sampling a human annotator from the population, the human annotator's choice of the preferred response is proportional to the response's utility value. Formally, we use $\prompt, \response_1,\response_2$ to denote the prompt and responses, the above interpretation implies the following assumptions:
\begin{assumption}[Existence of a Deterministic Oracle Utility Value]
    Given $\prompt$, the utility value of any response $\response$ exists and is deterministic. i.e., $\truereward_{\prompt,\response}, \forall \prompt,\response$ is a deterministic real value.
\end{assumption}
\begin{comment}
\begin{definition}[Individual Utility Evaluation Bias]
    For a \textbf{random} human annotator $A$, their evaluation of the utility value will deviate from the oracle utility value according to their individualized bias:
    \begin{equation}
        \truereward^{(A)}_{\prompt,\response} = \truereward_{\prompt,\response} + \annotatorbias(\prompt,\response,A),
    \end{equation}
    where $\annotatorbias(\prompt,\response,A)$ is a function over prompt $\prompt$, response $\response$, and annotator-dependent. Furthermore, we have 
    \begin{equation}
        \mathbb{E}_A \left[ \annotatorbias(\prompt,\response,A) \right] = 0, \forall \prompt,\response,
    \end{equation}
    and therefore
    \begin{equation}
        \mathbb{E}_A \left[ \truereward^{(A)}_{\prompt,\response} \right] = \truereward_{\prompt,\response}, \forall \prompt,\response,
    \end{equation}
\end{definition}
\ys{Note to self: this might not be compatible with logistic difference assumption}
\end{comment}
\begin{definition}[Individual Annotation under Bias]
    For annotator $A$, the annotation result is deterministic and depends on the comparison of their biased evaluation of the utility values of both responses $\response_1$ and $\response_2$, according to 
    \begin{equation}
        P_A(\response_1\succ \response_2 | \prompt) = \mathbbm{1}(\truereward^{(A)}_{\prompt,\response_1} > \truereward^{(A)}_{\prompt,\response_2}) = \mathbbm{1}\bigl(\truereward_{\prompt,\response_1} -\truereward_{\prompt,\response_2}  > \annotatorbias(\prompt,\response_1,A) - \annotatorbias(\prompt,\response_2,A) \bigr)
    \end{equation}
\end{definition}
Based on the above definitions, we can now explicitly write the assumption of applying the BT model to this randomized annotation process:
\begin{assumption}[Logistic Difference Assumption]
    The $\annotatorbias(\prompt,\response_1,A) - \annotatorbias(\prompt,\response_2,A)$ is sampled iid from a standard logistic distribution for all $\prompt,\response,A$:
    \begin{equation}
        P(\annotatorbias(\prompt,\response_1,A) - \annotatorbias(\prompt,\response_2,A) \le t) = \frac{1}{1+e^{-t}}
    \end{equation}
\end{assumption}
\begin{remark}(Transitive property of difference)
    A reader might be (rightfully) worried if this assumption is consistent with transitive property of difference, e.g., when considering multiple comparisons we have to have $\annotatorbias(\prompt,\response_{1},A)-\annotatorbias(\prompt,\response_3,A)=\annotatorbias(\prompt,\response_{1},A)-\annotatorbias(\prompt,\response_{2},A) + \annotatorbias(\prompt,\response_{2},A)-\annotatorbias(\prompt,\response_3,A)$ while knowing sum of (independent) logistic distributions is not logistic. One should be aware that the two terms being summed are not independent and the assumption can be achieved by assuming all annotator biases are independently Gumbel distributed with the same scale parameter.   
\end{remark}
With this assumption, we arrive at the BT-\textit{type} model
\begin{proposition}[BT-\textit{type} Model on Annotation under Logistic Difference Assumption]
    \begin{equation}
        P(\response_{1}\succ \response_{2} | \prompt) = P\bigl(\truereward_{\prompt,\response_{1}} -\truereward_{\prompt,\response_{2}}  > \annotatorbias(\prompt,\response_1,A) - \annotatorbias(\prompt,\response_2,A) \bigr) = \frac{1}{1+ e^{-(\truereward_{\prompt,\response_{1}} -\truereward_{\prompt,\response_{2}})}}
    \end{equation}
\end{proposition}
In comparison, we can alternatively have the following assumption and have another model:
\begin{assumption}[Gaussian Difference Assumption]
    The $\annotatorbias(\prompt,\response_1,A) - \annotatorbias(\prompt,\response_2,A)$ is sampled from a standard Gaussian distribution:
    \begin{equation}
        \annotatorbias(\prompt,\response_1,A) - \annotatorbias(\prompt,\response_2,A)\sim \mathcal{N}(0,1)
    \end{equation}
\end{assumption}
\begin{proposition}[Model on Annotation under Gaussian Difference Assumption]
    \begin{equation}
        P(\response_{1}\succ \response_{2} | \prompt) = P\bigl(\truereward_{\prompt,\response_{1}} -\truereward_{\prompt,\response_{2}}  > \annotatorbias(\prompt,\response_1,A) - \annotatorbias(\prompt,\response_2,A) \bigr) = \Phi(\truereward_{\prompt,\response_{1}} -\truereward_{\prompt,\response_{2}}),
    \end{equation}
    where $\Phi$ is the CDF of the Gaussian distribution.
\end{proposition}
%\begin{remark}(Assumption Self-Consistency)
%    We denote that this Gaussian difference assumption is self-consistent, and one way to achieve it is by having biases being Gaussian.
%\end{remark}
The next paragraph elaborates implications of those different assumptions.

\paragraph{Understanding the BT Model from a Gaussian Assumption on Players' Performance in a Game}
Technically, the BT model assumes that a player's ability \textbf{in a specific game} can be represented by a score. To better understand the rationale behind the BT model, we can take a step back and consider a Gaussian assumption for game performances. Specifically, we assume that in each two-player game, a player's performance can be modeled as a Gaussian distribution centered on their score, with the variance of these distributions capturing the stochastic nature of the game and the variability in the players' performances.

For instance, when player $A$ with a score of $S_A$ and variance $\sigma_A$ competes against player $B$ with a score of $S_B$ and variance $\sigma_B$, the probability that $A$ defeats $B$ in a game (denoted as $A \succ B$), given the Gaussian assumption on performance, is
\begin{equation}
\label{eqn:bt_prob}
    P(A \succ B) =P\left(x_a \ge x_b | x_a\sim N(S_A, \sigma_A^2), x_b\sim N(S_B, \sigma_B^2)\right) = \frac{1}{2} + \frac{1}{2}\mathrm{erf}\left(\frac{S_A-S_B}{\sqrt{2(\sigma_A^2+\sigma_B^2)}}\right).
\end{equation}
This is known to be the Thurstonian model~\citep{thurstone1927law}. In practice, if we further \textbf{assume} that the stochasticity characterized by performance variance is game-dependent rather than player-dependent, the denominator in \eqref{eqn:bt_prob} becomes a player-agnostic constant, which can be absorbed into the players' scores. In other words, \textbf{the absolute values in the scoring system are scaled by the inherent variability of the game.}

In the BT model, the $\mathrm{tanh}(\cdot)$ rather than the error function $\mathrm{erf}(\cdot)$ is used, for the sake of a better empirical fit and mathematical convenience.\footnote{So equivalently, the BT model assumes the players' performance differences are sampled from a logistic distribution rather than a Gaussian distribution.} Formally, the BT model is 
\begin{equation}
    \label{eqn:bt-model}
    P(A\succ B) = \frac{1}{1+e^{-(S_A - S_B)}}
\end{equation}

% \textcolor{red}{Data Generation: different types of data, how this is done in the literature. what type of data converges to the optimal embedding (linear models) fastest.}






% RLHF can be approached in two ways: The first approach is direct policy optimization~\cite{rafailov2024direct,zhao2023slic,azar2023general}, where the alignment of the LLM is achieved directly through single-stage supervised learning. The second approach involves first building a reward model, which is then used to guide the optimization of the LLM, either through supervised learning or reinforcement learning~\cite{yuan2023rrhf,dong2023raft,munos2023nash,li2023remax}. Despite differences in LLM alignment strategies, the majority of these methods --- including some of the most successful algorithms deployed for large-scale alignment tasks --- assume the BT model~\citep{bradley1952rank} to either explicitly or implicitly convert pairwise comparisons into scores, which are then used as objectives for the LLM to optimize.\footnote{In the standard application of the BT model, pairwise competition outcomes are converted into absolute scores that represent the players' abilities.}%\footnote{The BT model~\citep{bradley1952rank} and the Elo rating system~\citep{elo1978rating} were both developed for rating players in games originally.
% These methods convert pairwise competition outcomes into absolute scores that reflect the players' abilities.}




% \ys{A high-level comment: before going into the BT model, give a review on the setup of rank/score estimation: what are the data look like? Does the number of players diverge or stay constant? What is the goal there? Are evaluations done online or offline? If we'd use this to align LLM, what should be done (I remember @hs you once told me it needs online evaluations but we only have offline data)? Then go into Bradley Terry, then give another review on the setup of alignment with offline data, give a contrast to previous setting. One contribution, IMO, is to clear up these differences then proving consistency of a certain MLE. You need to convince other people what they might miss when using Bradley Terry in alignment settings.}
% \ys{I can try to clear things up a bit if there is a written-up on the two settings. I don't have enough material to work on in this section yet.}
% \jef{i agree with the above. From my perspective, the BT model is currently being chosen because of its easy implementation rather than its theoretical justification. In particular, if you look at the standard reward model training loss, it is nothing but a supervised learning procedure which "happens" to correspond to the BT model. This to me seems like the classic case of "let s throw NN into the problem and pray". However this in itself it not wrong, but what is wrong is that BT is usually used in cases where a player plays more than once i.e. think of a tennis tournament etc. In the classic reward model case, each player only plays once and hence, there is a clear disconnect between the BT setting and the preference data setting imo. What happens in reward modelling is that representation learning is happening and hence "good" samples get similar representations and "bad" samples get similar ones through extensive training. However this training is inefficient as the model needs to intrinsically learn this through data. Therefore, i believe having more structure in your preference data should effectively improve reward model learning. I give an example. Imagine, we have many preference pairs. However each of these pairs are comparisons between two bad samples. If we train BT on this data, the less bad samples i.e. winning samples get high scores. If we then add preference data between good and bad samples, the good samples get high score and the bad samples get low score. AT THE SAME TIME, the less bad samples from the first dataset will need to be pushed down again and hence there is some sort of "balancing act happening". If we had information on whether we are comparing two good or two bad or a good and a bad, that would intrinsically already make the training more efficient imo. This however is not the standard BT anymore and hence new methods should be proposed.}

==> tex/sec_dgp.tex <==
\newpage

\section{Rethinking Data Generation Processes for Reward Modeling}
\hs{Bradley Terry model is not the only notion of reward.}
\paragraph{Data Format}
We start our discussion with the classical preference dataset, which can be denoted as triples $\mathcal{D}_\mathrm{pref} = \{x_i, y^+_i, y^-_i\}_{i\in[N]}$, where $x_i\in \mathcal{X}$ is the prompt --- defined in the prompt space $\mathcal{X}$; and $y^+_i$ and $y^-_i$ are the preferred and dis-preferred responses, respectively --- defined in the response space $\mathcal{Y}$. 

\paragraph{Data Generation Process}
% It is worth mentioning the data-generation process of the pairwise annotation $\mathcal{D}_\mathrm{pref} = \{x_i, y^+_i, y^-_i\}_{i\in[N]}$ for our discussion. 
In LLM alignment, we assume there \textbf{exists an unknown deterministic oracle utility function} $\mathcal{R}^*:\mathcal{X}\times\mathcal{Y}\mapsto \mathbb{R}$, toward which we aim to optimize the LLMs. (i.e., the ultimate goal of alignment is to optimize this oracle utility function). 

In order to align LLMs without access to this oracle utility function, we need to \textbf{build a reward function as a proxy of the oracle utility function}. In the literature, this is always done by including human annotators --- who are believed to have this utility function in their mind --- to provide pairwise feedback between two LLM responses given different prompts. 

Formally, we use $\mathcal{H}:\mathcal{X}\times\mathcal{Y}\times\mathcal{Y}\mapsto \{-1,1\}$ to denote human annotators, given two responses sampled from the language model\footnote{we assume the LLM generation is stochastic by setting the generation temperature to be larger than 0.} $\ell$: $y_1, y_2 \sim \ell(x)$ for a specific prompt $x$
% \ys{If you mean $\ell$ is a distribution here, say that explicitly and tell people what you mean by $\sim$, say these two responses are sample independently (the current notation looks like a function)} 
\begin{equation}
    \mathcal{H}(x,y_1,y_2) = 
    \begin{cases} 
  1, & \text{if }~~ (y_1|x) \succ (y_2|x),\\
  -1, & \text{otherwise}
\end{cases}
\label{eq:annotator}
\end{equation}
% \ys{Just to double check, do we want 1/0 or $\pm 1$ for the sign thing?}\hs{because of the sigmoid function we used, normally people use +1, 0. }
where $(y_1|x) \succ (y_2|x)$ denotes that the annotator believes response $y_1$ given prompt $x$ is superior to $y_2$.
Since human annotators are not the oracle themselves, those preferences are only \textit{roughly} aligned with the oracle utility function, with some \textit{noises} injected --- limited by the ability to identify which is better. Different from the Bradley-Terry model where we assume the human preferences have individual level randomized biases, in this case we make the following assumption:
\begin{assumption}[Imperfect Preference Annotation in Approximating oracle\hs{TODO:download those references in psychology and read + confirm we can cite..}]\footnote{As has been demonstrated in the phchological literature~\citep{stewart2005absolute,guest2016relative}}
%%%%% More literature to be confirmed:
% Stewart, N., Brown, G. D., & Chater, N. (2005). "Absolute identification by relative judgment." Psychological Review, 112(4), 881–911. doi:10.1037/0033-295X.112.4.881.

% This paper discusses how humans often resort to relative judgment when distinguishing between similar stimuli, highlighting limitations in accurately ranking or identifying objects when the differences between them are small.
% Tversky, A., & Kahneman, D. (1974). "Judgment under Uncertainty: Heuristics and Biases." Science, 185(4157), 1124-1131. doi:10.1126/science.185.4157.1124.

% Although this paper is not solely focused on ranking, it discusses the biases and heuristics that can affect human judgment in uncertain scenarios, including cases where similar options are difficult to distinguish.
% Böckenholt, U. (2001). "Thresholds and Intransitivities in Pairwise Judgments: A Multinomial Logit Model." Journal of Mathematical Psychology, 45(3), 511–527. doi:10.1006/jmps.2000.1319.

% This paper explores the probabilistic nature of human judgments in ranking tasks, specifically when performance differences are subtle, leading to intransitivities or inconsistencies in rankings.
% Yaniv, I., & Schul, Y. (1997). "Elimination and inclusion procedures in judgment." Journal of Behavioral Decision Making, 10(3), 211-220. doi:10.1002/(SICI)1099-0771(199709)10:3<211::AID-BDM254>3.0.CO;2-6.

% This study discusses how human decision-making becomes more difficult when ranking similar objects and the cognitive strategies people employ in such scenarios.
%%%%%%%
\label{assumption:2.1}
When the oracle utilities of responses are similar, it would be more challenging for human annotators to differentiate the underlying oracle utility, formally,
\begin{equation}
    \mathrm{Prob}\left[\mathbbm{1} \bigl(\mathcal{H}_\beta(x,y_1,y_2) = \sign (\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x) ) \bigr) \bigg|  \big|\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)\big| = \Delta r \right] = \sigma(\beta \Delta  r),
\end{equation}
where $\beta>0$ characterizes the ability of annotators, and $\sigma$ is the sigmoid function. \textcolor{blue}{More generally, $\sigma$ can be replaced by any monotonic differentiable function valued 0.5 at 0 and 1 at positive infinity.}

\begin{remark}[Differences between Assumption \ref{assumption:2.1} and the Bradley-Terry Model Assumption]
    \hs{TODO: (make this more rigorous:) To apply the Bradley-Terry model, we need to attribute the stochasticity in annotations to the randomized biases, and then explicitly assume the responses' utility differences are sampled from a logistic distribution. This is a wild assumption. But in our order consistency framework, we have Assumption 2.1, which is much easier to be verified in practice (really?).}
\end{remark}
% \ys{Give some intuition here on this assumption. I assume you are saying that the probability of the annotator giving the true ranking is based on the utility difference between the two responses.}

% \ys{I'm unsure $\mathcal{R}^*$ is defined. Is it the true utility function $\mathcal{R}^*$ or the noisy version of the annotator (given later on you assumed a distribution on it)? I assume you mean the true one but things are random later. I also assume by $\sigma$ you mean sigmoid, this is not necessarily good since you use $\sigma$ for variance of normal later on. }

% \ys{How do you handle equal sign? Do you assume the utility function has the property that $\mathcal{R}^*(y_1)=\mathcal{R}^*(y_2)$ implies $y_1=y_2$?}
\end{assumption}
\begin{definition}[Optimal and Random Annotator]
    The annotators' ability to identify better responses from the worse concerning the oracle utility is characterized by the parameter $\beta$. Specifically, when $\beta \xrightarrow{}\infty$, $\mathcal{H}_\beta\xrightarrow{}\mathcal{H}^*$ becomes the \textbf{optimal annotator} and probability of correct annotation 
    % $$\mathrm{Prob}\left[\mathcal{H}_\beta(x,y_1,y_2) = \mathbbm{1}\bigl(\mathcal{R}^*(y_1|x) >  \mathcal{R}^*(y_2|x) \bigr) \bigg|  \big|\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)\big| = \Delta r \right]  \xrightarrow{\beta \xrightarrow{} \infty} 1.$$ 
    $$
    \mathrm{Prob}\left[\mathbbm{1} \bigl(\mathcal{H}_\beta(x,y_1,y_2) = \sign (\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x) ) \bigr) \bigg|  \big|\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)\big| = \Delta r \right] \xrightarrow{\beta \xrightarrow{} \infty} 1.
    $$
    Similarly, we can define the \textbf{random annotator} when $\beta=0$, and the probability of correct annotation becomes:
    % $$\mathrm{Prob}\left[\mathcal{H}_\beta(x,y_1,y_2) = \mathbbm{1}\bigl(\mathcal{R}^*(y_1|x) >  \mathcal{R}^*(y_2|x) \bigr) \bigg|  \big|\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)\big| = \Delta r \right] \xrightarrow{\beta \xrightarrow{} 0} 0.5.$$ 
    $$
    \mathrm{Prob}\left[\mathbbm{1} \bigl(\mathcal{H}_\beta(x,y_1,y_2) = \sign (\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x) ) \bigr) \bigg|  \big|\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)\big| = \Delta r \right] \xrightarrow{\beta \xrightarrow{} 0} 0.5
    $$
\end{definition}
Importantly, those two responses are randomly sampled from a single LLM $\ell$ by increasing its generation stochasticity. We assume the oracle utility of those two responses are sampled from a Gaussian distribution with mean $\mu_x$ and variance $\sigma^2_x$, i.e., 
$$
y\sim\ell(x), \mathcal{R}^*(y|x)\sim \mathcal{N}(\mu_x, \sigma_x^2 ),
$$
where the subscript $x$ denotes the mean values and variances' dependence on the prompts. 
\begin{definition}[Annotation Order Consistency
%\ys{I would call this accuracy instead of consistency, consistency (in statistics term) often involve some asymptotics and here you are talking about finite sample metric}
]
    For prompt $x$, responses $y_1, y_2$, we say the annotation given by annotator $\mathcal{H}_\beta$ to be \textbf{order-consistent} if $\mathcal{H}_\beta (x, y_1, y_2) (\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)) \ge 0$ 
    % \ys{this is a random variable, do you mean $\ge 0$ all the time? So you are saying the annotator can tell which one is greater correctly?}
    . Correspondingly, we define the annotation order consistency on $y_1, y_2$ given $x$ as a random variable
    \begin{equation}
    \label{eqn:annotation_consistency}
        \mathbbm{1}\left(\mathcal{H}_\beta (x, y_1, y_2) (\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)) \ge 0\right)
    \end{equation}
\end{definition}

\begin{restatable}[Average Order Consistency of Annotation]{proposition}{PropAvgQuality}
\label{prop:1}
    When data for pairwise annotation is generated through random sampling of two responses $y_1, y_2 \sim \ell(x)$, the annotation quality $\mathcal{Q}^\beta_\mathrm{pair}$ can be defined as the averaged annotation order consistency:
    \begin{equation}
    \begin{split}
         \mathcal{Q}_\mathrm{pair} = \mathbb{E}_{y_1,y_2|x}[ \tau_x ]
         % &= \mathbb{E}_{x}\left[  \mathbbm{1}\left(\mathcal{H}_\beta (x, y_1, y_2) (\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)) \ge 0\right)
         % \right]\\
         % &= \mathbb{E}_{x}\left[ \mathrm{Prob}\left(\mathcal{H}_\beta(x,y_1,y_2)= \mathbbm{1}(\mathcal{R}^*(y_1|x) >  \mathcal{R}^*(y_2|x))\right) \right] \\
         &= \mathbb{E}_{y_1,y_2|x}\left[ \sigma(\beta|\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)|) \right] %\\ 
         % &, 
    \end{split}
    \end{equation}
    % \ys{Be explicit on what this expectation is taking over, I assume you mean condition on $x$ and marginalize $y$}
    where $\tau_x= \sigma(\beta|\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)|)$ is a random variable (over $y_1, y_2$) and the probability density function of $\tau_x $ is 
    \begin{equation}
        % f(\tau) = \frac{1}{\sqrt{\pi \sigma_x^2}} \exp\left(-\frac{\left(\log\left(\frac{\tau}{1-\tau}\right)\right)^2}{4\sigma_x^2}\right) \cdot \frac{1}{\tau(1-\tau)}
        f_{\tau_x}(t) = \frac{1}{\sqrt{\pi \beta^2\sigma_x^2}} \exp\left(-\frac{\left(\log\left(\frac{t}{1-t}\right)\right)^2}{4\beta^2\sigma_x^2}\right) \cdot \frac{1}{t(1-t)}
    \end{equation}
\end{restatable}
% \ys{There is no way this thing is true per definition of $\tau$ \cref{eqn:annotation_consistency}. Remember that $\tau$ is an indicator function and thus binary. It should not have a PDF w.r.t. Lebesgue as shown here. What you show here is the distribution of $\mathbb{E}_{x}[ \tau ]$ marginalize over $y$ condition on $x$, be careful about what is random in your statement.}
Proof is provided in Appendix~\ref{appdx:proof_prop1}

\begin{remark}[Numerical Results.]
    When $\beta^2\sigma_x^2 = 1$, we can get a numerical results $\mathcal{Q}_{\mathrm{pair}}\approx 0.6749$, e.g., roughly $67.5\%$ of data are correctly labeled by annotators.
    Similarly, when $\beta^2\sigma_x^2 = 2$, $\mathcal{Q}_{\mathrm{pair}}\approx 0.7251$; when $\beta^2\sigma_x^2 = 4$, $\mathcal{Q}_{\mathrm{pair}}\approx 0.7781$; when $\beta^2\sigma_x^2 = 10$, $\mathcal{Q}_{\mathrm{pair}}\approx 0.8428$; 
\end{remark}


\begin{mdframed}[innertopmargin=6pt,leftmargin=0pt, rightmargin=0pt, innerleftmargin=10pt, innerrightmargin=10pt, skipbelow=0pt]
\textbf{Interpretations: }  
This \textcolor{red}{suggests} that the effect of better annotators and the effect of response utility diversity are always coupled: in order to improve data quality, we may either improve the ability of annotators or further diversify the generation utilities --- as both of those parameters control the annotation quality. However, this entanglement tells us that without further assumption, it is \textbf{impossible to disentangle the annotators' ability from the prompt-relevant variance of response utilities.} 
\end{mdframed}

\jef{Let's try to formalize this a little bit more. I am not sure if we can draw such strong interpretations from the above. We can chat about this later.}
\ys{I agree...}

\begin{graybox}[innertopmargin=0pt]
\paragraph{Research Opportunities:} 
This reveals several open questions to be researched further: 
\begin{enumerate}[leftmargin=*,nosep]
    \item (Data-Centric Research) How to improve the data generation process to incorporate more information in the labeling and avoid the aleatoric uncertainty due to imperfect annotation? The analysis above hints at the possibility of enhancing the diversity of utility. 
    \item (Algorithm-Centric Research) Given the above data generation process (as common practice in the literature), what are the properties of different reward model estimators when trying to recover the unknown oracle utility function $\mathcal{R}^*$?
\end{enumerate}
\end{graybox}

In the next section, we will focus on the second question and try to draw theoretical insights into building reward model estimators.




==> tex/sec_ensemble.tex <==


\newpage
\section{Practical Reward Model Ensemble at Scale}
By separating the representation learning phase of the reward model, it would be easy to scale up reward model ensembles. 




==> tex/sec_rm_estimators.tex <==

% \newpage
% \section{Rethinking Learning Objectives for Reward Modeling}
% \subsection{The Pair-Binary Classification (PBC) Objective}

% \begin{equation}
% \label{eq:pair_clf_obj}
%     \mathcal{L}_\mathrm{PBC} (\theta) = -\mathbb{E}_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}}\left[\log 
% \left(\sigma(R^\mathrm{PBC}_\theta(x,y^+,y^-)\right) - \log 
% \left( 1 - \sigma(R^\mathrm{PBC}_\theta(x, y^-,y^+))\right)\right]
% \end{equation}

% Without loss of generality, we can disentangle the representation (embedding) learning and reward model learning by denoting the reward model $R^\mathrm{PBC}_\theta$ to be a linear function over a representation function $\phi$, i.e., $R^\mathrm{PBC}_\theta(x,y^+,y^-) = w_\mathrm{PBC}^T \phi(x,y^+,y^-)$, we have
% \begin{equation}
% \label{eqn:deriv_pbc}
%     \frac{\partial \mathcal{L}_{PBC}}{\partial w} = E_{y^+, y^-} \left[ -\left(1 - \sigma(w_\mathrm{PBC}^T \phi(x,y^+,y^-))\right) \phi(x,y^+,y^-) + \sigma(w_\mathrm{PBC}^T \phi(x,y^-,y^+)) \phi(x,y^-,y^+) \right] = 0
% \end{equation}

% Moreover, it would be natural to impose $R^\mathrm{PBC}_\theta(x,y^+,y^-) = - R^\mathrm{PBC}_\theta(x,y^-,y^+)$ as an additional constraint over the reward function given the symmetric property of $R^\mathrm{PBC}$. Therefore, we can further simplify Equation (\ref{eqn:deriv_pbc}) to
% \begin{equation}
%     \frac{\partial \mathcal{L}_{PBC}}{\partial w} = E_{y^+, y^-} \left[ -\left(1 - \sigma(w_\mathrm{PBC}^T \phi(x,y^+,y^-))\right) \phi(x,y^+,y^-) \right] = 0
% \end{equation}



% \subsection{The Bradley Terry Objective}
% On the other hand, building on the Bradley-Terry model, the learning objective of a pairwise preference dataset is given by 
% \begin{equation}
% \label{eq:bt_obj}
%     \mathcal{L}_\mathrm{BT} (\theta) = -\mathbb{E}_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}}\left[\log \sigma 
% \left(R^\mathrm{BT}_\theta(x, y^+) - R^\mathrm{BT}_\theta(x, y^-)\right)\right]
% \end{equation}

% Similarly, denoting $R^\mathrm{BT}_\theta$ as a linear function over a representation function $\phi$, i.e., $R^\mathrm{BT}_\theta(x,y) = w_\mathrm{BT}^T \phi(x,y)$, we have

% \begin{equation}
% \label{eqn:deriv_bt}
%     \frac{\partial L_{BT}}{\partial w} = E_{y^+, y^-} \left[ -(1-\sigma( w_\mathrm{BT}^T(\phi(x,y^+) - \phi(x,y^-))  ) ) (\phi(x,y^+) - \phi(x,y^-)) \right] = 0
% \end{equation}

% Comparing Equation (\ref{eqn:deriv_bt}) and Equation (\ref{eqn:deriv_pbc}), we see \textcolor{blue}{the Bradley-Terry reward model is a special instantiation of the PBC reward model, where the symmetry is explicitly imposed through $R^\mathrm{PBC}_\theta(x,y^+,y^-) = R^\mathrm{BT}_\theta(x,y^+) - R^\mathrm{BT}_\theta(x,y^-)$}
% \subsection{The Binary Classification (BC) Objective}

% \begin{equation}
% \label{eq:clf_obj}
%     \mathcal{L}_\mathrm{BC} (\theta) = -\mathbb{E}_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}}\left[\log 
% \left(\sigma(R^\mathrm{BC}_\theta(x, y^+)\right) - \log 
% \left( 1 - \sigma(R^\mathrm{BC}_\theta(x, y^-))\right)\right]
% \end{equation}

% In this case, denoting $R^\mathrm{BC}_\theta$ to be a linear function over representations, we have $R^\mathrm{BC}_\theta(x,y) = w_\mathrm{BC}^T \phi(x,y)$ and 
% \begin{equation}
%     \frac{\partial \mathcal{L}_{BC}}{\partial w} = E_{y^+, y^-} \left[ -\left(1 - \sigma(w_\mathrm{BC}^T \phi(x, y^+))\right) \phi(x, y^+) + \sigma(w_\mathrm{BC}^T \phi(x, y^-)) \phi(x, y^-) \right] = 0
% \end{equation}


% \subsection{\textcolor{red}{Which Objective Shines with What Dataset?}}
% \textcolor{red}{can we discuss some properties of those different learning objectives?}


==> tex/sec_rm_target.tex <==
\section{Approximating oracle Utility with Imperfect Annotations}
\subsection{Preference Model Learning through Order Consistency Maximization}
 % \ys{ This title reads like you are gonna show your optimization results will converge to some true thing as more data being collected}
In LLM alignment, the objective of reward modeling is to learn a proxy preference model that is \textit{aligned} with the oracle utility function $\mathcal{R}^*$, such that in the inference (test) time, we can use this learned preference model to optimize the generation (or optimize the model through e.g., rejection sampling~\citep{dong2023raft}). %In general, there are two types of ranking models we could consider: (1) reward model --- that maps prompt-response tuple $(x,y)$ into a score; or (2) preference model --- that maps prompt-response pair triples $(x,y_1,y_2)$ into binary;

% In such a process, we would like to ask the question:

% \textbf{\textit{How to best estimate $\mathcal{R}^*$, using the noisy partial observations in $\mathcal{D}_\mathrm{pref} = \{x_i, y^+_i, y^-_i, (p^*_i)\}_{i\in[N]}$, where $(p^*_i)$ is the hidden variable denoting the probability of getting a correct label.}}

In such a process, we highlight the principled property of optimizing \textbf{\textit{order consistency}}. e.g., in annotation, the objective of improving its quality could be quantified through \eqref{eqn:annotation_consistency}. Similarly, in preference model learning, we can formally define the estimation order consistency as follows:

\begin{definition}[Preference Estimator Order Consistency]
    For prompt $x$, responses $y_1, y_2$, we say a preference estimator $\hat{H}_\theta$ --- parameterized by $\theta$ --- to be consistent with regard to $\mathcal{H}_\beta$ if $\hat{H}_\theta(x, y_1, y_2)\mathcal{H}_\beta (x, y_1, y_2)\ge 0$. Correspondingly, we define the estimator's order consistency on $x, y_1, y_2$ as a random variable
    \begin{equation}
    \label{eqn:annotation_consistency}
        \tau_{\hat{H}_\theta} = \mathbbm{1}\left(\hat{H}_\theta(x, y_1, y_2)\mathcal{H}_\beta (x, y_1, y_2)\ge 0\right)
    \end{equation}
\end{definition}

In our work, we propose to learn preference estimators by maximizing the expected preference estimation order consistency: %\ys{What's the range of $\hat H$? $\mathcal{H}_\beta$ is binary so I guess all $H$'s are binary? Or is it difference in utility function?}\hs{we can decide weather to put constraints or not to the range of $H$} \ys{follow up question: since $H_\beta$ is 0 or 1 why do we want sign consistency ($\hat{H}_\theta(x, y_1, y_2)\mathcal{H}_\beta (x, y_1, y_2)\ge 0$ says they are the same sign)?}
\begin{equation}
\label{eqn:learning_obj}
    \max_{\theta \in \Theta} \mathbb{E}_{x, y_1,y_2 \sim \ell(x)} \left[ \mathbbm{1}\left(\hat{H}_\theta(x, y_1, y_2)\mathcal{H}_\beta (x, y_1, y_2)\ge 0\right) \right].
\end{equation}
This learning objective is motivated by the following proposition, in the sense that given an actual distance between two utility values, if we can have the objective~\eqref{eqn:learning_obj} arbitrarily close to 1, we can have control the population level error with high probability. %\ys{I think this is the motivation but there is a gap here, we can only optimize population level loss, not conditioning on distance between $y_1$, $y_2$, which means it is possible that this loss is dominated by pairs that has very distance utility rather than ambiguity ones. In the theorem we need to condition on the distance between pairs, which is NOT the objective} 

%\ys{It might be a larger gap than I initally expected since how well $\hat H$ approximate $H_\beta$ implicitly depends on the true utility difference between $y_1$ and $y_2$, it can be the case that it is extremely well when this distance is small and horrible when it is large, which can lead to a good objective (since we averaged over all possible distances) but bad performance when r is big when testing (but we might have a large probability bound) I initially thought we can just use Markov inequality to control the conditional probability but I'm unsure how to handle the event that in some r $\hat H$ having bad approximation. The case is that when this approximation is right the annotator is bad and when annotator is good the approximation is wrong. By the objective itself we cannot uniformly control error over all $r$. Here is a cooked up example for this problem, suppose there is $\epsilon$ chance the distance between $y_1$ $y_2$ denoted by $r$ being 1000 and $1-\epsilon$ chance $r=0$, when $r=0$ we have $\hat H=H_\beta$ and when $r=1000$ we ask $\hat H=1-H_\beta$, it's overall objective function is very good $1-\epsilon$ but majority of the time we are just randomly guessing}
% \begin{theorem}
%     \textcolor{red}{Prove something like if the above objective is optimized, then $\hat{H}$ and the oracle reward is also optimized with respect to consistency?}
% \end{theorem}

\begin{restatable}[Order Consistency Lower Bound]{proposition}{ThmO}
\label{theorem1}
Given annotator ability \(\beta > 0\), condition on true utility difference \(\Delta r := |\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)|\), and the annotator function \(\mathcal{H}_\beta(x, y_1, y_2)\) provides feedback that probabilistically aligns with the oracle utility \(\mathcal{R}^*(x, y)\) according to:
    \begin{equation}
    \mathrm{Prob}\left(\mathcal{H}_\beta(x, y_1, y_2) = \mathbbm{1}(\mathcal{R}^*(y_1|x) > \mathcal{R}^*(y_2|x))\bigg|  \Delta r\right) = \sigma(\beta \Delta r),
    \end{equation}
    % where \(\mathcal{R}^*(y|x) = \mathcal{R}^*(x, y)\) and \(\sigma(\cdot)\) any monotonic function to $[0.5, 1]$. When the learned model \(\hat{H}_{\theta^*}(x, y_1, y_2)\). Suppose objective~\eqref{eqn:learning_obj} is well defined and can be optimized to $1-\delta\epsilon$ for some small $\delta$ and $\epsilon<3/20$, i.e., we have 
    where \(\mathcal{R}^*(y|x)\) is the unknown oracle utility function, and \(\sigma(\cdot)\) any monotonic function to $[0.5, 1]$. Suppose the learned model \(\hat{H}_{\theta^*}(x, y_1, y_2)\) is obtained by optimizing objective~\eqref{eqn:learning_obj} to $1-\delta\epsilon$ for some small $\delta$ and $\epsilon<3/20$, i.e., we have 
    \begin{align}
        \mathbb{E}_{x, y_1,y_2 \sim \ell(x)} \left[ \mathbbm{1}\left(\hat{H}_{\theta^*}(x, y_1, y_2)\mathcal{H}_\beta (x, y_1, y_2)\ge 0\right) \right]\ge 1-\delta\epsilon
    \end{align}
%\ys{I'll rewrite the proof first, the statement is not ready yet}    

Then, with probability at least $1-\delta$ over $\Delta r$, for a given $\Delta r$ the order consistency of \(\hat{H}_{\theta^*}\) with respect to the oracle utility is bounded below by:
\begin{equation}
\begin{split}
\label{eqn:oracle_util_order_con_obj}
    &\mathbb{E}_{x, y_1, y_2 \sim \ell(x)}\left[\mathbbm{1}\left(\hat{H}_{\theta^*}(x, y_1, y_2)(\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)) \geq 0\right)\bigg|  \Delta r\right] \\
    &\geq (1 - \epsilon) \cdot \sigma^2(\beta \Delta r) + \epsilon \cdot (1 - \sigma(\beta \Delta r))^2 \\ 
    &= \sigma^2(\beta \Delta r) - (2\sigma(\beta \Delta r) - 1) \epsilon 
\end{split}
\end{equation}

Further if we assume that with probability at least $1-\kappa$, that $\sigma(\beta \Delta r)\ge \sqrt{\epsilon^2+1-3\epsilon}+\epsilon$, we have
\begin{align}
    \mathbb{E}_{x, y_1, y_2 \sim \ell(x)}\left[\mathbbm{1}\left(\hat{H}_{\theta^*}(x, y_1, y_2)(r^*(y_1|x) - r^*(y_2|x)) \geq 0\right)\right]\geq 1-4\epsilon-\kappa-\delta
\end{align}
\ys{Do we want this bound to be a $1-\epsilon$ bound? we can make it by change $\delta$ and $\epsilon$ in the assumptions. I like the current version better in the sense it is easier to parse and follow proofs. The current result is probably the best we can do since most of the bounds used are sharp}
%\ys{$\xi$ can be $4\epsilon$ if this new notation annoys us}
\end{restatable}
\begin{remark}[Works with perfect annotator]
    For a perfect annotator with $\beta = \infty$, we have the second assumption always hold if $P(\Delta r=0)=0$ and our objective directly controls the population approximation quality.
\end{remark}
%\ys{Move forward to fix this gap: assume something about the tail of $\Delta r$ thus $\sigma(\beta \Delta r)$, union bound 1) $\Delta r$ too small and 2) reward model being unreliable and combine all things to get a high probability bound}

\begin{comment}
\begin{restatable}[Order Consistency Lower Bound]{theorem}{ThmOne}
\label{theorem1}
Given annotator ability \(\beta > 0\), and the annotator function \(\mathcal{H}_\beta(x, y_1, y_2)\) provides feedback that probabilistically aligns with the oracle utility \(\mathcal{R}^*(x, y)\) according to:
    \begin{equation}
    \mathrm{Prob}(\mathcal{H}_\beta(x, y_1, y_2) = \mathbbm{1}(\mathcal{R}^*(y_1|x) > \mathcal{R}^*(y_2|x))) = \sigma(\beta |\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)|),
    \end{equation}
    where \(\mathcal{R}^*(y|x) = \mathcal{R}^*(x, y)\) and \(\sigma(\cdot)\) is the logistic sigmoid function. When the learned model \(\hat{H}_{\theta^*}(x, y_1, y_2)\) differs from the annotator model \(\mathcal{H}_\beta(x, y_1, y_2)\) with probability at most \(\epsilon\):
    \begin{equation}
     \mathrm{Prob}\left(\mathrm{sign}(\hat{H}_{\theta^*}(x, y_1, y_2)) \neq \mathrm{sign}(\mathcal{H}_\beta(x, y_1, y_2))\right) \leq \epsilon.
    \end{equation}

Then, the order consistency of \(\hat{H}_{\theta^*}\) with respect to the oracle utility is bounded below by:
\begin{equation}
\begin{split}
\label{eqn:oracle_util_order_con_obj}
    &\mathbb{E}_{x, y_1, y_2 \sim \ell(x)}\left[\mathbbm{1}\left(\hat{H}_{\theta^*}(x, y_1, y_2)(\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)) \geq 0\right)\right] \\
    &\geq (1 - \epsilon) \cdot \sigma^2(\beta \Delta r) + \epsilon \cdot (1 - \sigma(\beta \Delta r))^2 \\ 
    &= \sigma^2(\beta \Delta r) - (2\sigma(\beta \Delta r) - 1) \epsilon 
\end{split}
\end{equation}
where \(\Delta r = |\mathcal{R}^*(y_1|x) - \mathcal{R}^*(y_2|x)|\). %\ys{My sanity check is to send $\delta r\to 0$ and I expect things to be something around .5 but we got .25}
\end{restatable}

Proof is provided in Appendix~\ref{appdx:proof_theorem1}. 
\begin{remark}[Monotonicity]
    Equation (\ref{eqn:oracle_util_order_con_obj}) is monotonic increasing function over $\sigma$, and monotonic decreasing function over $\epsilon$. Hence either improving the annotation quality or improving the preference estimator's order consistency will tighten the above lower bound.
\end{remark}
\end{comment}
The takeaway message from Proposition \ref{theorem1} is that optimizing the order consistency between the preference estimator and the human annotator also optimizes the order consistency between the preference estimator and the oracle utility function. \ys{If the annotator has good ability, optimizing this objective controls population level error rate of preference.}
%\ys{You basically said that an approximation (learned function) of an approximation (noisy utility from annotator) is not bad when both steps are good enough. } \hs{Aug.24: can we further generalize the above theorem to more general functions? @ys}\ys{It's a bound on ways things fail so it should be pretty much general to all functions, your proof does not rely on any of the properties of $\sigma$ nor $H$. }
\jef{this bound looks interesting but we have to be aware that the delta term might be vaccuous, Also if i understand correctly, the quantity with $\theta*$ is always above or equal to zero to begin with?}

\subsection{Choices of Parameterization in Practical Optimization}
In practice, the learning objective of \eqref{eqn:learning_obj} can be rewritten through tagging the responses such that we use $y^+$ to denote $y_1$ if $\mathcal{H}_\beta(x,y_1,y_2)>0$, else $y^+ = y_2$ and $y^- = y_1$. 
With finite sample annotation provided by human annotators, we estimate the expectation using empirical sample mean:
% \ys{there is a leap here, how is the $\mathcal{H}_\beta$ term dropped?} \hs{I changed the notation into $y^+, y^-$, such that $\mathcal{H}_\beta$ is always 1.} \ys{Then say in practice we only have access to samples $y^+_{(n)}$, $y^-_{(n)}$ and we estimate this expectation using empirical mean, by the tagging mechanism we always have $\mathcal{H}_\beta=1$, and the sample version of that population objective is what you wrote below. If it is an empirical mean you wanna be explicit about it, it it is done by an SGD it is an approximation of an approximation. alternatively you can be explict that this expectation is taken over the empirical distribution of x y+ y- rather than their population version. }
\begin{equation}
\label{eqn:simplified_obj}
    \max_{\theta \in \Theta} \sum_{(x, y^+,y^-)\sim \mathcal{D}_\mathrm{pref}} \left[ \mathbbm{1}\left(\hat{H}_\theta(x, y^+, y^-) \ge 0\right) \right].
\end{equation}


\jef{i agree that this objective is good to learn. the questions that is currently not clearly answered is how this will be used later on. Having such an estimator needs to be incorporated into the LLM alignment process later on. We need to think: 1. is there any benefit of this over standard reward models and 2. Can we trivially use this estimator into RLHF (with some modifications) or can we possibly come up with a training scheme from the RL literature if 1. indeed shows benefits.} \ys{my intuition here is that 1) binary data is not information rich to estimate an continuous function 2) at the end of the day we only care about the best response rather than their actual utility value which does not need we to get continuous utility function out 3) dealing with binary estimand is much easier variance-wise. I think we can show some estimation variance estimate and apply some concentration inequality}
In this work, we study three different parameterization choices as instantiations of the preference models. It is worth noting that in all instantiations, we enforce the estimator to have the symmetry property to regularize the estimation.
\ys{Need to tell me what $\theta$'s and $R_\theta$'s are}

\paragraph{Direct Paired Preference Model (Paired-Train, Paired-Call, \textit{PTPC})} 

    PTPC is the most straightforward parameterization, yet it suffers from inference-time efficiency difficulty. Because it can only provide pairwise comparisons, it has an $O(n\log n)$ time complexity on average.
    \begin{equation}
        \hat{H}_\theta(x, y^+, y^-) = R_{\theta_\mathrm{PTPC}}(x, y^+, y^-),
    \end{equation}
    Using the sigmoid function $\sigma$ to convert the parameterized reward into probability $\sigma(R_{\theta_\mathrm{PTPC}}):\mathbb{R}\mapsto\Delta(\{0,1\})$, the maximum likelihood estimation loss given observational data is 
    \begin{equation}
    \label{eq:pair_clf_obj_no_symmetry}
        \mathcal{L}^\mathrm{MLE}_\mathrm{PTPC} (\theta) = -\sum_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}}\left[\log 
    \left(\sigma(R_{\theta_\mathrm{PTPC}}(x,y^+,y^-)\right) + \log 
    \left( 1 - \sigma(R_{\theta_\mathrm{PTPC}}(x, y^-,y^+))\right)\right]\footnote{In the equation, the second term is introduced to avoid the trivial solution where the labels are encoded in input position.}.
    \end{equation}
    % \textit{Avoid Encoding Labels in Input Positions:}  
    
    We assume we can disentangle the representation (embedding) learning and reward model learning by denoting the reward model $R_{\theta_\mathrm{PTPC}}$ to be a linear function over a representation function $\phi$, i.e., $R_{\theta_\mathrm{PTPC}}(x,y^+,y^-) = w_\mathrm{PTPC}^T \phi(x,y^+,y^-)$, we have
    
   \begin{equation}
    \label{eqn:deriv_pbc}
    \begin{split}
        &\frac{\partial \mathcal{L}^\mathrm{MLE}_\mathrm{PTPC} (\theta)}{\partial w} = 0 \\
        &= \sum_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}} \bigl[ -\left(1 - \sigma(w^T \phi(x, y^+, y^-))\right) \phi(x, y^+, y^-) + \sigma(w^T \phi(x, y^-, y^+)) \phi(x, y^-, y^+) \bigr] .
    \end{split}
    \end{equation}

Furthermore, if we impose the constraint of symmetry into the parameterization of $\hat{H}_\theta$ through 
    \begin{equation}
        \hat{H}_\theta(x, y^+, y^-) = R_{\theta_\mathrm{PTPC}}(x, y^+, y^-) - R_{\theta_\mathrm{PTPC}}(x, y^-, y^+)
    \end{equation}
Let \( \Delta\phi(x, y^+, y^-) = \phi(x, y^+, y^-) - \phi(x, y^-, y^+) \). The gradient equation, set to zero, simplifies to:

\begin{equation}
    \frac{\partial \mathcal{L}^\mathrm{MLE}_\mathrm{PTPC} (\theta)}{\partial w} =\sum_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}} \left[\left(\sigma\left(w^T \Delta\phi(x, y^+, y^-)\right) - 1\right) \cdot \Delta\phi(x, y^+, y^-)\right] = 0.
\end{equation}

\paragraph{Decomposed Preference Model (Paired-Train, Isolated-Call, \textit{PTIC})}
    Another parameterization method is the Pairwise Training with Isolated Comparison (PTIC), which preserves the symmetry property by independently estimating the values of both responses. This approach allows for efficient inference-time ranking with an \( O(n) \) complexity, hence significantly improving scalability with respect to the number of inference-time responses.

    \begin{equation}
        \hat{H}_\theta(x, y^+, y^-) = R_{\theta_\mathrm{PTIC}}(x, y^+) - R_{\theta_\mathrm{PTIC}}(x, y^-).
    \end{equation}
    
    Again, using the sigmoid function \( \sigma \) to convert the reward into probability, the Maximum Likelihood Estimation (MLE) loss given the observational data is defined as:
    \textcolor{red}{What is the difference between this one and the BT model motivation?}
    \begin{equation}
        \mathcal{L}^\mathrm{MLE}_\mathrm{PTIC} (\theta) = -\sum_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}}\left[\log \left(\sigma\left(R_{\theta_\mathrm{PTIC}}(x, y^+) - R_{\theta_\mathrm{PTIC}}(x, y^-)\right)\right)\right].
    \end{equation}

This loss function seeks to maximize the likelihood that the model correctly predicts the preference between two responses by using the difference in their isolated estimated values. 

To compute the gradient of the MLE loss with respect to the parameter vector \( w \), assuming the reward function is linear in \( w \) (i.e., \( R_{\theta_\mathrm{PTIC}}(x, y) = w^T \phi(x, y) \)), the gradient is:

\begin{equation}
    \frac{\partial \mathcal{L}^\mathrm{MLE}_\mathrm{PTIC} (\theta)}{\partial w} = \sum_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}} \left[\left(\sigma\left(w^T (\phi(x, y^+) - \phi(x, y^-))\right) - 1\right) \cdot \left(\phi(x, y^+) - \phi(x, y^-)\right)\right].
\end{equation}

    
    
\paragraph{Direct Binary Classification Model (Isolated-Train, Isolated-Call, \textit{ITIC}). }
    
In this case, we consider a tightened variant of \eqref{eqn:simplified_obj} to impose a more stringent constraint in preference learning. Although this objective is more restrictive than the original, it allows us to achieve $O(n)$ time complexity and enables learning with non-pairwise data using off-the-shelf binary classification algorithms.\footnote{This approach offers greater flexibility compared to the previous method, which relied solely on MLPs in instantiation 2.} The refined objective is expressed as:
    \begin{equation}
        \begin{split}
            & \max_{\theta \in \Theta} \mathbb{E}_{x, y^+,y^-} \left[ \mathbbm{1}\left(\hat{H}_\theta(x, y^+, y^-) \ge 0\right) \right] \\ 
            % &= \max_{\theta \in \Theta} \mathbb{E}_{x, y^+,y^-} \left[ \mathbbm{1}\left(R_{\theta_\mathrm{Dec}}(x, y^+) - R_{\theta_\mathrm{Dec}}(x, y^-) \ge 0\right) \right] \\ 
            &\ge \max_{\theta \in \Theta} \mathbb{E}_{x, y^+,y^-} \left[ \mathbbm{1}\left(R_{\theta_\mathrm{ITIC}}(x, y^+)\ge 0\right)\mathbbm{1}\left(R_{\theta_\mathrm{ITIC}}(x, y^-) \le 0\right) \right]
        \end{split}
    \end{equation}

The MLE loss given observational data is defined as:

\begin{equation}
    \mathcal{L}^\mathrm{MLE}_\mathrm{ITIC}(\theta) = -\mathbb{E}_{x, y^+, y^-} \left[ \log \sigma\left(R_{\theta_\mathrm{ITIC}}(x, y^+)\right) + \log \left(1 - \sigma\left(R_{\theta_\mathrm{ITIC}}(x, y^-)\right)\right) \right],
\end{equation}

Assuming the reward function is linear in \( w \) (i.e., \( R_{\theta_\mathrm{PTIC}}(x, y) = w^T \phi(x, y) \)), the gradient of the loss with respect to \( w \) is given by:

\begin{equation}
    \frac{\partial \mathcal{L}^\mathrm{MLE}_\mathrm{ITIC}(\theta)}{\partial w} = \mathbb{E}_{x, y^+, y^-} \left[\left(1 - \sigma\left(w^T \phi(x, y^+)\right)\right) \phi(x, y^+) - \sigma\left(w^T \phi(x, y^-)\right) \phi(x, y^-)\right].
\end{equation}

    
% \paragraph{\textcolor{red}{KTO --- I'm planning to remove the discussion on KTO as it is a direct alignment method. (i.e., no explicit reward model learning.)}}

\subsection{Convergence Rate of Estimators}
\textcolor{red}{TODO: variance control using concentration inequality.}
\ys{All three seems to be M-estimators, there are classic theories on them, should be thinking more about distribution of embeddings}

\section{Generalized Variance Comparison of PTPC, PTIC, and ITIC Estimators}

\hs{TODO: [WHEN To USE Which? Bound related to data variance --- like prompt variance] I'm reading the Doubly Robust paper and other literature in OPE (especially on the contextual bandit settings) and hopefully we can adapt some theorems on estimation variance / biases from there. --- i.e., we are now studying doubly robust methods in preference-based learning without BT, previous methods can not do this due to the unclear BT assumption (is this true? -- what was the previous challenge in studying doubly robust methods in reward modeling?).}



% \newpage
% \section{Optimization of Preference Models toward Consistency}
% \subsection{The Pair-Binary Classification (PBC) Objective}

% \begin{equation}
% \label{eq:pair_clf_obj}
%     \mathcal{L}_\mathrm{PBC} (\theta) = -\mathbb{E}_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}}\left[\log 
% \left(\sigma(R^\mathrm{PBC}_\theta(x,y^+,y^-)\right) - \log 
% \left( 1 - \sigma(R^\mathrm{PBC}_\theta(x, y^-,y^+))\right)\right]
% \end{equation}

% We assume we can disentangle the representation (embedding) learning and reward model learning by denoting the reward model $R^\mathrm{PBC}_\theta$ to be a linear function over a representation function $\phi$, i.e., $R^\mathrm{PBC}_\theta(x,y^+,y^-) = w_\mathrm{PBC}^T \phi(x,y^+,y^-)$, we have
% \begin{equation}
% \label{eqn:deriv_pbc}
%     \frac{\partial \mathcal{L}^\mathrm{MLE}_\mathrm{PTPC} (\theta)}{\partial w} = \mathbb{E}_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}} \left[ -\left(1 - \sigma(w^T \phi(x, y^+, y^-))\right) \phi(x, y^+, y^-) + \sigma(w^T \phi(x, y^-, y^+)) \phi(x, y^-, y^+) \right] = 0
% \end{equation}

% Moreover, it would be natural to impose $R^\mathrm{PBC}_\theta(x,y^+,y^-) = - R^\mathrm{PBC}_\theta(x,y^-,y^+)$ as an additional constraint over the reward function given the symmetric property of $R^\mathrm{PBC}$. Therefore, we can further simplify Equation (\ref{eqn:deriv_pbc}) to
% \begin{equation}
%     \frac{\partial \mathcal{L}_{PBC}}{\partial w} = E_{y^+, y^-} \left[ -\left(1 - \sigma(w_\mathrm{PBC}^T \phi(x,y^+,y^-))\right) \phi(x,y^+,y^-) \right] = 0
% \end{equation}



% \subsection{The Bradley Terry Objective}
% On the other hand, building on the Bradley-Terry model, the learning objective of a pairwise preference dataset is given by 
% \begin{equation}
% \label{eq:bt_obj}
%     \mathcal{L}_\mathrm{BT} (\theta) = -\mathbb{E}_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}}\left[\log \sigma 
% \left(R^\mathrm{BT}_\theta(x, y^+) - R^\mathrm{BT}_\theta(x, y^-)\right)\right]
% \end{equation}

% Similarly, denoting $R^\mathrm{BT}_\theta$ as a linear function over a representation function $\phi$, i.e., $R^\mathrm{BT}_\theta(x,y) = w_\mathrm{BT}^T \phi(x,y)$, we have

% \begin{equation}
% \label{eqn:deriv_bt}
%     \frac{\partial L_{BT}}{\partial w} = E_{y^+, y^-} \left[ -(1-\sigma( w_\mathrm{BT}^T(\phi(x,y^+) - \phi(x,y^-))  ) ) (\phi(x,y^+) - \phi(x,y^-)) \right] = 0
% \end{equation}

% Comparing Equation (\ref{eqn:deriv_bt}) and Equation (\ref{eqn:deriv_pbc}), we see \textcolor{blue}{the Bradley-Terry reward model is a special instantiation of the PBC reward model, where the symmetry is explicitly imposed through $R^\mathrm{PBC}_\theta(x,y^+,y^-) = R^\mathrm{BT}_\theta(x,y^+) - R^\mathrm{BT}_\theta(x,y^-)$}
% \subsection{The Binary Classification (BC) Objective}

% \begin{equation}
% \label{eq:clf_obj}
%     \mathcal{L}_\mathrm{BC} (\theta) = -\mathbb{E}_{(x,y^+,y^-) \sim \mathcal{D}_\mathrm{pref}}\left[\log 
% \left(\sigma(R^\mathrm{BC}_\theta(x, y^+)\right) - \log 
% \left( 1 - \sigma(R^\mathrm{BC}_\theta(x, y^-))\right)\right]
% \end{equation}

% In this case, denoting $R^\mathrm{BC}_\theta$ to be a linear function over representations, we have $R^\mathrm{BC}_\theta(x,y) = w_\mathrm{BC}^T \phi(x,y)$ and 
% \begin{equation}
%     \frac{\partial \mathcal{L}_{BC}}{\partial w} = E_{y^+, y^-} \left[ -\left(1 - \sigma(w_\mathrm{BC}^T \phi(x, y^+))\right) \phi(x, y^+) + \sigma(w_\mathrm{BC}^T \phi(x, y^-)) \phi(x, y^-) \right] = 0
% \end{equation}


% \subsection{\textcolor{red}{Which Objective Shines with What Dataset?}}
% \textcolor{red}{can we discuss some properties of those different learning objectives?}




% \section{Future Work of This Paper}
% \textbf{Part 2 (ICLR/AISTATS: optional experiment section of this paper)}

% In part 1, we justified binary classifiers can be used in building reward models, thus enabling leveraging off-the-shelf classification algorithms on top of embedding data to improve (1) learning stability (2) performance (3) inference time delay (4) memory and computation (5) scalability of ensemble.

% In our experiments, we verify those 5 properties by highlighting the superiority of tree-based models --- XGBoost, which has achieved widely success in tabular data.  



% \textbf{Part 3 (ICML: Online RLHF: Data-Centric RLHF research with our stable reward modeling algorithms.)}

% After justifying the above properties of reward modeling, we further explore how to adapt those techniques to real-world large-scale alignment systems. Specifically, we study the ``exploration" problem in RLHF to maximally utilize the limited budget of annotation and improve the sample complexity (w.r.t. number of annotations) in online alignment. 

% It is worth noting that, this part of research is highly dependent on the stability provided by our tree-based reward model. Otherwise, with the conventional Bradley-Terry-based reward model, the training instability causes large variance and it would be extremely difficult to draw conclusions and insights from noisy experimental observations.

